Is Learning Effective in Dynamic Strategic Interactions? Evidence from Stackelberg Games

In many settings of interest, a policy is set by one party, the leader, in order to influence the action of another party, the follower, where the follower's response is determined by some private information. A natural question to ask is, can the leader improve their strategy by learning about the unknown follower through repeated interactions? A well known folk theorem from dynamic pricing, a special case of this leader-follower setting, would suggest that the leader cannot learn effectively from the follower when the follower is fully strategic, leading to a large literature on learning in strategic settings that relies on limiting the strategic space of the follower in order to provide positive results. In this paper, we study dynamic Bayesian Stackelberg games, where a leader and a \emph{fully strategic} follower interact repeatedly, with the follower's type unknown. Contrary to existing results, we show that the leader can improve their utility through learning in repeated play. Using a novel average-case analysis, we demonstrate that learning is effective in these settings, without needing to weaken the follower's strategic space. Importantly, this improvement is not solely due to the leader's ability to commit, nor does learning simply substitute for communication between the parties. We provide an algorithm, based on a mixed-integer linear program, to compute the optimal leader policy in these games and develop heuristic algorithms to approximate the optimal dynamic policy more efficiently. Through simulations, we compare the efficiency and runtime of these algorithms against static policies.

==> contract.tex <==
\section{Application to Dynamic Contract Design}

In this section, we discuss a specific principal-agent problem known as the contract design problem, in order to illustrate the implications of our previous results. What is more, by utilizing certain structural properties of the contract design game, we are able to show more intriguing outcomes regarding the characteristics of dynamic principal policies. 

The agent has $[n] = \{1, \cdots, n\}$  actions to choose from. Each action $j \in [n]$ results in a probabilistic distribution $\p_j \in \Delta^m$ over $[m]=\{1,\cdots, m\}$ outcomes and has a corresponding cost $c_j \in \rr_{+}$. Therefore, every agent's type $\theta$ is determined by the matrix $P \in \rr^{n \times m}$ together with the cost vector $\c \in \rr^n$. On the other hand, the principal has a reward $r_i \in \rr_+$ for every outcome $i \in [m]$. The principal designs contract $\x \in \rr^m_+$ which specifies payment $x_i$ to the agent if outcome $i$ is realized. As a result, the principal's utility function can be computed as follows.
\begin{equation}\label{eq:contract_principal}
U(\x, j) = \sum_i (r_i - x_i) p_{j, i} = R_j - \langle \x, \p_j \rangle,
\end{equation}
where $R_j = \sum_i r_i p_{j, i}$ denotes the expected reward for action $j \in [n]$. The agent's utility function is denoted as follows.
\begin{equation}\label{eq:contract_agent}
V^\theta(\x, j) = \langle \x, \p_j \rangle - c_j.
\end{equation}

%Consistent with the existing literature, 
As standard assumptions in the contract design model \citep{dutting2019simple,alon2021contracts,castiglioni2021bayesian},  we assume the first outcome has zero rewards for the principal and this outcome only occurs if and only if the agent takes the first action, which has zero cost as well. In addition, there are no actions that can be considered ``dominated'', meaning that for any two actions $j$ and $j'$, their expected rewards $R_j$ and $R_{j'}$ are distinct and the action with a higher expected outcome ($R_j > R_{j'}$) also incurs a higher cost ($c_j > c_{j'}$). There is a unique action $j^*$ that maximizes the welfare, i.e., $j^* = \argmax_j R_j - c_j.$ Next, we show that there exists a compact representation of the optimal dynamic  policy to the leader utilizing the structural assumption on the contra design problem. 
\begin{theorem}\label{thm:compact}
Computing the optimal dynamic contract is a problem in NP. That is, there always exists an optimal dynamic contract (as the certificate for the decision version of the problem) that has description size   $ \text{poly}(m,n,T,|\Theta|).$ %can be represented with a description size of $O\big(\text{poly}(m,n,T,|\Theta|)\big).$
\end{theorem}
\begin{proof}
For any optimal dynamic contract (i.e. the $\DSE$, $\x^*$ and $\j^*$, which forms an optimal solution to \eqref{eq:u_l^DySS}), there exists a best response path $\j^{*\theta}_T$ for every type $\theta \in \Theta$. Also, note that the description size of $\x^*$ is $O(n^{T}m)$ since $\x^*$ needs to specify the principal contract for any possible agent action history. Next, we propose to construct a dynamic $\hat{\x}$ that only needs polynomial description size but achieves the same expected principal revenue as $\x^*$. Specifically, for any round $t \in [T]$ and for any possible agent action history $\j_{t-1}$, we construct $\hat{\x}^t_{\j_{t-1}}$ as follows.
\begin{enumerate}
    \item If there exists $\theta \in \Theta$ such that $\j_{t-1} = \j^{*\theta}_{t-1}$, then we set $\hat{\x}^t_{\j_{t-1}} = \x^{*t}_{\j_{t-1}}$.
    \item Otherwise, set $\hat{\x}^t_{\j_{t-1}} = \bvec{0}$, i.e. does not pay the agent anything.
\end{enumerate}
Note that the dynamic contract $\hat{\x}$ only specifies contract for $|\Theta|$ types of action paths (denoted as $J_T$), where each path has a length of $T$. As a result, the above dynamic contract only has a description size of $O(mT|\Theta|)$. Next, we show that $\hat{\x}$ achieves the same expected revenue for the principal, which is equivalent to showing that every agent type $\theta$ follows the same response path under $\hat{\x}$ and $\x^*$. Given a dynamic contract $\x$ and follower response history $\j_T$, we denote the follower's cumulative utility as 
\[
V^\theta(\x, \j_T) = \sum_{t \in [T]} \sum_{i \in [m]} x^t_{j_{t-1},i} \, p^\theta_{j_t,i} - c^\theta_{j_t} 
\]
Next, we consider the following two cases for any follower type $\theta$.

For any path $\j_T \in J_T$ and $\j_T \ne \j^{*\theta}_T$, we have \begin{equation}\label{eq:first_case}V^\theta(\x^*, \j_T^{*\theta}) \ge V^\theta(\x^*, \j_T) = V^\theta(\hat{\x}, \j_T)\end{equation}  by the incentive compatibility of $\x^*$ and the definition of $\hat{\x}$. 

For any path $\j_T \notin J_T$, there must exist a time step $\hat{t} \le T$ such that $j_{t} = 0$ for all $\hat{t} \le t \le T$, and $\hat{t}$ represents the time step when the leader discovers the $\j_T \notin J_T$ and does not pay the agent (i.e. $\hat{\x}^t = \bvec{0}$ for all $\hat{t} \le t \le T$). First of all, we still have $V^\theta(\x^*, \j_T^{*\theta}) \ge V^\theta(\x^*, \j_T)$ by the incentive compatibility of $\x^*$. In addition, we have 
\[
V^\theta(\hat{\x}, \j_T) = \sum_{t=1}^{\hat{t} - 1} \sum_{i = 1}^m \hat{x}^t_{j_{t-1},i} \, p^\theta_{j_t,i} - c^\theta_{j_t} = \sum_{t=1}^{\hat{t} - 1} \sum_{i = 1}^m x^{*t}_{j_{t-1},i} \, p^\theta_{j_t,i} - c^\theta_{j_t}
\]
by the definition of $\hat{\x}$. Next, we show  $V^\theta(\x^*, \j_T^{*\theta}) \ge V^\theta(\hat{\x}, \j_T)$.
\begin{equation}\label{eq:second}
    \begin{split}
        V^\theta(\x^*, \j_T^{*\theta}) &= \sum_{t=1}^{T} \sum_{i = 1}^m x^{*t}_{j^{*\theta}_{t-1},i} \, p^\theta_{j^{*\theta}_t,i} - c^\theta_{j^{*\theta}_t} %+ \sum_{t=\hat{t}}^{T} \sum_{i = 1}^m x^{*t}_{j^{*\theta}_{t-1},i} \, p^\theta_{j^{*\theta}_t,i} - c^\theta_{j^{*\theta}_t} \\
        %&\overset{(i)}{\ge} \sum_{t=1}^{\hat{t} - 1} \sum_{i = 1}^m x^{*t}_{j^{*\theta}_{t-1},i} \, p^\theta_{j^{*\theta}_t,i} - c^\theta_{j^{*\theta}_t} \\
        \overset{(i)}{\ge}\sum_{t=1}^{\hat{t} - 1} \sum_{i = 1}^m x^{*t}_{j_{t-1},i} \, p^\theta_{j_t,i} - c^\theta_{j_t} \\
        & = \sum_{t=1}^{\hat{t} - 1} \sum_{i = 1}^m \hat{x}^t_{j_{t-1},i} \, p^\theta_{j_t,i} - c^\theta_{j_t} = V^\theta(\hat{\x}, \j_T)
    \end{split}
\end{equation}
Note the inequality $(i)$ is by the fact that $\j^{*\theta}_T$ is optimal for the follower. Suppose $(i)$ does not hold, then we can come up with a follower response sequence, which plays $j_1, \cdots, j_{t-1}$ for the first $\hat{t} - 1$ rounds followed by non-effort actions (i.e. the action with $0$ utility for the agent) afterward, contradicting the optimality $\j^{*\theta}_T$. 

Combing \eqref{eq:first_case} and \eqref{eq:second}, we show that it is still optimal for the follower type $\theta$ to follow the path $\j_T^{*\theta}$ under the contract $\hat{\x}$, proving that $\hat{\x}$ achieves the same expected principal utility as $\x^*$.
\end{proof}

%\noindent As a result, Theorem \ref{thm:compact} shows that the decision problem for $\DSE$ of dynamic contract design is in NP, and is NP-complete. 
In line with our previous outcomes concerning generalized principal-agent problems, we present practical algorithms to address the optimal dynamic contracts and Markovian contracts utilizing $\MILP$.

\begin{corollary}
    The optimal dynamic Markovian  contract can be computed by a $\MILP$ with a $O(T|\Theta|mn^2)$ number of continuous variables and $T|\Theta|n$ integer variables; The exact $\DSE$ can be computed by a $\MILP$ with a $O(T|\Theta|mn^T)$ number of continuous variables and $T|\Theta|n$ integer variables.
\end{corollary}

This result is directly implied by Theorem \ref{thm:Markovian_policy} and Proposition \ref{prop:program_equivalent}. For example, We can substitute the previous utility functions of the principal and the agent with equations \eqref{eq:contract_principal} and \eqref{eq:contract_agent} and get the following $\MILP$ for computing the $\DSE$ for dynamic contract design games.

\begin{maxi}[2]<b>{}{\sum_{t\in[T]} \sum_{\theta \in \Theta}\mu(\theta) \sum_{\j_t \in [n]^t} \sum_{i\in[m]} p^\theta_{j_t,i}(r_i z^{t,\theta}_{\j_t} - w^{t,\theta}_{\j_t,i})}{}{}
\addConstraint{\textstyle \sum_{t' \in [t]} y^\theta_{t', j_{t'}} - t+1 \le z^{t,\theta}_{\j_t}}{\leq y^\theta_{t', j_{t'}}, }{\forall \j_t \in [n]^t, t' \in [t], t \in [T], \theta \in \Theta}
\addConstraint{w^{t,\theta}_{\j_t, i} \le x^t_{\j_{t-1},i}; \,  w^{t,\theta}_{\j_t, i}  \le z^{t,\theta}_{\j_t}; \, w^{t,\theta}_{\j_t, i} \ge x^t_{\j_{t-1},i} - (1-z^{t,\theta}_{\j_t})M, \,\,}{}{\forall \j_t \in [n]^t, t \in [T], \theta \in \Theta, i \in [m]}
\addConstraint{\textstyle 0 \le a_\theta - \big(\sum_{t, i}  x^t_{\j_{t-1},i} \, p^\theta_{j_t,i} - c^\theta_{j_t}\big)}{\le M(T - \sum_t y^\theta_{t, j_{t}}), \,\,}{\forall \j_T \in [n]^T, \theta \in \Theta}
\addConstraint{\textstyle \sum_j y^\theta_{t, j}}{= 1,\labelOP{OP:MILP}}{\forall t \in [T], \theta \in \Theta}
\addConstraint{0 \le \w; \quad 0 \le \x; \quad 0 \le \z \le 1; \quad \y \in \{0, 1\}}{}{}
\end{maxi}

Similar to Theorem \ref{thm:infinte_T}, we can show that the dynamic contract is provably nearly optimal even relative to stronger static strategy spaces for the principal that allow for such things as communication between the principal and the agent. We also have a specific contract design example, which shows $\RME$ will be $\Omega(1)$ worse than the average $\DSE$ utility, even when there is only a single agent type.

Consider the following contract design example.
\begin{table}[H]
\begin{center}
\begin{small}
\begin{subtable}{0.4\linewidth}
    \centering
    \begin{tabular}{|c|c|c|} \hline
      $P$  &  $o_1$ & $o_2$  \\ \hline
      $a_0$   & 0 & 0 \\ \hline
      $a_1$   & 0.5 & 0.5 \\ \hline
      $a_2$   & 0 & 1 \\ \hline
    \end{tabular} 
\end{subtable}
\end{small}
\end{center}
\caption{An example contract design game, where $P$ denotes each agent's action $a_j$'s ($j \in \{0, 1, 2\}$) probabilistic distribution over outcomes $\{o_1, o_2\}$. Each action $a_i$ has a corresponding cost vector $c_i$ and the agent's cost vector is $\c =[0, 0.1, 0.3]$. In addition, every outcome $o_1/o_2$ has a corresponding reward $0.5/1$ for the principal.}
\label{table:contract}
\end{table}

It can be computed that the optimal single-round contract for the principal is to design a contract as $\x=(0, 0.2)$, i.e. pay the agent with  payment $0.2$ is outcome $o_2$ is realized, resulting in a utility of $0.65$ for the principal where the agent responds by playing action $a_1$.

On the other hand, for any $T > 1$, the principal can design the contract as follows:
\begin{equation}\label{eq:dy_contract}
\x^{t} = (0, 0),\, \forall t=1, \cdots, T-1;\quad  \x^T = \begin{cases}(0, 0.3T) \quad \text{if $j_t = a_2 \,\,\forall t<T$} \\ (0, 0) \quad \text{otherwise}\end{cases}.
\end{equation}
As a result, the agent will always play action $a_2$, resulting in a total utility of $0.7 T$. There is a gap $0.05 T$ between the total principal utility under the optimal static contract and the dynamic contract \eqref{eq:dy_contract}, equivalently $\Omega(1)$ gap between the average $\DSE$ utility and $\RME$ utility.

Note that in the example of Table \ref{table:contract}, the principal can extract the maximal full surplus from the agent (i.e., pay the agent the exact amount of cost he spent such that the agent gets zero utility). It turns out that this is not a coincidence. Next, we show that the principal is always able to extract the maximal full surplus from the agent utilizing the special structural property of the contract design game. 
%\begin{assumption}[
%Existence of Dominated Payment 
% \begin{definition}[Inducibility Gap of Welfare-Maximizing Action \mh{payment dominance region}]\label{assump:dominated_payment}
% For a contract design instance, let $j^* = \argmax_{j} R_j - c_j$ be the agent action that achieves the maximal welfare, and the inducibility gap of welfare-maximizing action is defined as \[\textstyle \Delta^* = \max_{\x\in\{\x:\|\x\|\le 1\}} \min_{j \not = j^*} \sum_i x_i(P_{j^*,i} - P_{j,i}) .\] 
% %We assume there exists $x^*$ such that \[\textstyle \quad \sum_i x^*_i(P_{j^*,i} - P_{j,i}) \ge 0, \,\, \forall j \ne j^*.\]
% \end{definition}
\begin{definition}[Payment-dominance Region and Ratio]\label{assump:dominated_payment}
%For a contract design instance, l
Let $j^* = \argmax_{j} R_j - c_j$ be the agent action that achieves the maximal welfare. The payment dominance region  $X^*$ is defined as the set of all contracts whose expected pay on $j^*$ is strictly more than that of any other action, or formally, \[\textstyle X^* =  \{ \x: \sum_i x_i(P_{j^*,i} - P_{j,i}) > 0, \forall j \not = j^* \};\]
The payment dominance ratio $\q(\x)$ for any $\x \in X^*$ is defined as 
\[
q_j(\x) = \frac{\sum_i x_i P_{j^*, i}}{\sum_i x_i (P_{j^*, i} - P_{j, i})} \quad \forall j\ne j^*.
\]
%We assume there exists $x^*$ such that \[\textstyle \quad \sum_i x^*_i(P_{j^*,i} - P_{j,i}) \ge 0, \,\, \forall j \ne j^*.\]
\end{definition}

\noindent Non-emptiness of the payment dominance region $X^*$ guarantees the existence of   a contract such that its expected payment of playing the action $j^*$, which  maximizes the social welfare, is greater than the expected payment of other actions.  With this definition, we are ready to show that the principal is always able to extract the maximal social welfare (i.e., $\max_j R_j - c_j$) with a dynamic contract when $T$ is large enough and the principal knows the agent's utility function.

\begin{proposition}
    For any contract design instance with non-empty payment-dominance region $X^*$, the  optimal dynamic contract   extracts  full surplus within  any interaction period $T \geq T_0$ where
    \[T_0 = \big\lceil  \min_{\x \in X^*} \,  \max_{j \in \{j:  c_{j} < c_{j^*}\}} q_j(\x)(1-c_j/c_{j^*})  \big\rceil  \] is an instance-dependent parameter that depends on the  payment-dominance ratio.  
    % and if $\{j': c_{j^*} > c_{j'}\} = \emptyset$, we can further simply the interaction period as follows.
    % \[T \ge \min_{\x \in X^*}  \frac{\sum_i x_i P_{j^*, i}}{c_{j^*}}.\]
    %\frac{\alpha\sum_i x^*_iP_{j^*,i}}{c_{j^*}},\]
    %\[T\ge \frac{\alpha\sum_i x^*_iP_{j^*,i}}{c_{j^*}},\] 
    %where 
    %$\alpha = \max_{j \in \{j': c_{j^*} > c_{j'}\}} \frac{c_{j^*}-c_j}{\sum_i x^*_i(P_{j^*,i} - P_{j,i})}$,
    % $\alpha = \max\big(0, \max_j \frac{c_{j^*}-c_j}{\sum_i x^*_i(P_{j^*,i} - P_{j,i})}\big)$, 
    %and $\x^*$ is any principal contract that has a positive $\Delta^*$. \mh{change positive to positive} %\hf{can we characterize $T$ in term of the $\Delta^*$ above?}\hf{why we need to emphasize the following? I thought all your model assumes this? }when the principal knows the agent's utility function.
\end{proposition}

\noindent   Note that the set $\{j:  c_{j} < c_{j^*}\}$ is always non-empty, since $\argmin_j c_j$ cannot be $j^*$ due to its social welfare being $0$ as defined. Next, we will demonstrate the construction of such a dynamic contract.
%We remark that 

\begin{proof}
Denote $j^* = \argmax_{j\in[n]} \sum_i P_{j, i} r_i - c_j$, i.e. the agent action that achieves the maximal welfare. We propose the following contract to extract the first-best surplus from the agent.
\begin{equation}\label{eq:dy_contract_general}
\x^{t} = \bvec{0},\, \forall t=1, \cdots, T-1;\quad  \x^T = \begin{cases} \x^* \quad \text{if $j_t = j^* \,\,\forall t<T$} \\ \bvec{0} \quad \text{otherwise}\end{cases}. 
\end{equation}
where $\x^*$ satisfies the following linear system:
\begin{equation}\label{eq:optimal_contract}
    \begin{split}
    &\sum_i P_{j^*,i} x^*_i = Tc_{j^*}; \\
    &\sum_i P_{j,i} x^*_i \le (T-1) c_{j^*} + c_j, \quad\forall j \ne j^*.
    \end{split}
\end{equation}
or equivalently,
\begin{equation}\label{eq:another_format}
\begin{split}
 &\sum_i P_{j^*,i} x^*_i = Tc_{j^*}; \\
    &\sum_i x^*_i(P_{j^*,i} - P_{j,i}) \ge c_{j^*} - c_j, \quad\forall j \ne j^*.
\end{split}
\end{equation}
By definition \ref{assump:dominated_payment} of $X^*$, for any $\hat{\x} \in X^*$, it satisfies the following property:%there exists a $\hat{\x}$ such that  
%\[\textstyle \sum_i \hat{x}_iP_{j^*,i} \ge c_{j^*} \quad \text{and} \quad 
\[\sum_i \hat{x}_i(P_{j^*,i} - P_{j,i}) > 0, \,\, \forall j \ne j^*.\]

\noindent Next, we prove there always exists a $\x^*$ that satisfies \eqref{eq:another_format} by construction.
First of all, we must have $\sum_i \hat{x}_i(P_{j^*,i} - P_{j,i}) \ge c_{j^*}-c_j$ if $c_{j^*} \le c_j$. 
On the other hand,  for the actions $j \in \{j': c_{j^*} > c_{j'}\}$ let $\alpha = \min_{j \in \{j': c_{j^*} > c_{j'}\}} \frac{\sum_i \hat{x}_i(P_{j^*,i} - P_{j,i})}{c_{j^*}-c_j}$ and we define $\bar{\x} = \hat{\x}/\alpha$. Thus we have 
\[
\sum_i \bar{x}_i(P_{j^*,i} - P_{j,i}) = \frac{\sum_i \hat{x}_i(P_{j^*,i} - P_{j,i})}{\alpha} \ge {\textstyle \sum_i \hat{x}_i(P_{j^*,i} - P_{j,i})} \frac{c_{j^*}-c_j}{\sum_i \hat{x}_i(P_{j^*,i} - P_{j,i})}  = c_{j^*}-c_j,
\]
where the inequality is by definition of $\alpha$. As a result, we have $\bar{\x}$ satisfies the \textit{second} constraint of \eqref{eq:another_format}. 
%If $\alpha \ge 1$, then we have $\hat{\x}$ satisfies the second constraint of \eqref{eq:another_format} since $\sum_i \hat{x}_i(P_{j^*,i} - P_{j,i}) \ge c_{j^*}-c_j$ for all $j \ne j^*$; Otherwise, we let $\bar{\x} = \hat{\x}/\alpha$ (i.e. $\bar{\x} = \hat{\x} /\min(1,\alpha)$) and we have $\bar{\x}$ satisfies the \textit{second} constraint of \eqref{eq:another_format} as well.

Finally, we construct $\x^*$, which satisfies \textit{both} constraints of \eqref{eq:another_format}, based on $\bar{\x}$. 
%we note that we always have $\sum_i \bar{x}_iP_{j^*,i} \ge c_{j^*}$ since $\bar{\x} = \hat{\x} /\min(1,\alpha)$. 
If  $\sum_i \bar{x}_iP_{j^*,i} = T c_{j^*}$ for some natural number $T \in \nn=\{1,2,3,\cdots\}$, we already have the existence of $\x^*=\bar{\x}$ that is feasible to \eqref{eq:another_format}. On the other hand, if  $\sum_i \bar{x}_iP_{j^*,i} \ne T c_{j^*}$, we let $\x^* = T \frac{c_{j^*}}{\sum_i \bar{x}_iP_{j^*,i}} \bar{\x}$ where $T \in \nn$. Thus, we have \[\sum_i P_{j^*,i} x^*_i = Tc_{j^*} \frac{\sum_i \bar{x}_iP_{j^*,i}}{\sum_i \bar{x}_iP_{j^*,i}} = T c_{j^*}.\] To make sure $\x^*$ still satisfies the second constraint of \eqref{eq:another_format}, we must have $T$ is large enough such that $T  \ge \frac{\sum_i \bar{x}_iP_{j^*,i}}{c_{j^*}}$ (i.e., $T \frac{c_{j^*}}{\sum_i \bar{x}_iP_{j^*,i}} \ge 1$), which guarantees the left-hand side values (positive for all $j \ne j^*$) of the second constraint of \eqref{eq:another_format} increase. As a result, we have shown the existence of $\x^*$ when \[T\ge \frac{\frac{1}{\alpha} \sum_i \hat{x}_iP_{j^*,i}}{c_{j^*}} = \max_{j \in \{j': c_{j^*} > c_{j'}\}} \frac{\sum_i \hat{x}_i P_{j^*, i}}{\sum_i \hat{x}_i(P_{j^*,i} - P_{j,i})} (1-c_j/c_{j^*}) = \max_{j \in \{j': c_{j^*} > c_{j'}\}} q_j(\hat{\x})(1-c_j/c_{j^*}),\] where $\hat{\x}$ is any feasible strategy in $X^*$. Minimizing over $\hat{\x} \in X^*$ completes the proof of the proposition.
\end{proof}

==> model.tex <==


% \hf{Let's define Dynamic Stackelberg Equilibrium (\DySE) as the optimal \DySS, and then say we are computing DySE. Similarly, use BSE and MDSE and MRSE. \mh{seems to have too many notations.}}
% \hf{Take a look at this paper "Zero-Sum Stochastic Stackelberg Games" https://openreview.net/pdf?id=SWEgdj5k6e9, and its related works. See how they relate to us.  } \mh{Two main differences between \cite{goktas2022zero} and us: (1) we do not have stochastic structure (2) they study recursive Stackelberg equilibrium, which is a stationary policy.}

